On Smooth Combinatorial Products of Simplices

We show that every lattice weak Minkowski summand of a smooth polytope combinatorially isomorphic to a product of simplices has a quadratic triangulation. This is achieved by identifying this class of polytopes with the class of Nakajima polytopes. We combine these results to give a new proof that two lattice weak Minkowski summands of the same such smooth polytope are relatively IDP. Along the way, we prove a structure theorem for simple polytopes whose 2-faces are triangles and trapezoids.

==> tikz_diagrams/semidirectproduct.tex <==

\begin{tikzpicture}[line join=round, line cap=round, thick]

%% ---- P = triangle (flat arrowhead) ----
\begin{scope}[shift={(0,6)}]
  \node at (-1.2, 0) {$P \ =$};
  \coordinate (A) at (0, 0);   
  \coordinate (B) at (-0.9, -0.8); 
  \coordinate (C) at (1.8, 0); 
  \draw (A) -- (B) -- (C) -- cycle;
  \fill[gray!50] (A) -- (B) -- (C) -- cycle;
\end{scope}

%% ---- Q = vertical line segment ----
\begin{scope}[shift={(6,6)}]
  \node at (-0.8, 0) {$Q \ =$};
  \draw (0, -0.6) -- (0, 0.6);
\end{scope}

%% ---- 
\begin{scope}[shift={(2.4,3.3)}]
  \node at (-2, 0.5) {$Q \rtimes P \ =$};

  % Bottom triangle
  \coordinate (A) at (0, 0);   
  \coordinate (B) at (-0.9, -0.8); 
  \coordinate (C) at (1.8, 0); 
  \draw (A) -- (B) -- (C) -- cycle;
  \fill[gray!50] (A) -- (B) -- (C) -- cycle;

  % Top triangle
  \coordinate (D) at (0, 1.2);   
  \coordinate (E) at (-0.9, 1.6); 
  \coordinate (F) at (1.8, 1.5); 
  \draw (D) -- (E) -- (F) -- cycle;
  \fill[gray!20] (D) -- (E) -- (F) -- cycle;

  % Top to bottom edges (should be parallel)
  \draw (A) -- (D);
  \draw (B) -- (E);
  \draw (C) -- (F);

\end{scope}

%% ---- Q \ltimes P 
\begin{scope}[shift={(2.2,0.3)}]
  \node at (-2.8, 0.5) {$P \rtimes Q \ =$};

  % Bottom triangle
  \coordinate (A) at (0, 0);   
  \coordinate (B) at (-0.9, -0.8); 
  \coordinate (C) at (1.8, 0); 
  \draw (A) -- (B) -- (C) -- cycle;
  \fill[gray!50] (A) -- (B) -- (C) -- cycle;

  % Top triangle
  \coordinate (D) at (0, 1.5);   
  \coordinate (E) at (-1.8, 0.3); 
  \coordinate (F) at (3.6, 1.5); 
  \draw (D) -- (E) -- (F) -- cycle;
  \fill[gray!50] (D) -- (E) -- (F) -- cycle;

  % Top to bottom edges (should be parallel)
  \draw (A) -- (D);
  \draw (B) -- (E);
  \draw (C) -- (F);
  
\end{scope}

\end{tikzpicture}

